Exploring Website Location as a Security Indicator

Authenticating websites is an ongoing problem for users. Recent proposals have suggested strengthening current server authentication methods by incorporating website location as a comprehensible additional trust factor. In this work, we explore users' acceptance of location information and how it affects decision-making for security and privacy. We conducted a series of qualitative interviews to learn how location can be integrated into users' decision-making for security, and we designed a security indicator to alert the user to changes in website locations. We evaluated our tool in a 44-participant user study and found that users were less likely to perform security-sensitive tasks when alerted to location changes. Our results suggest that website location can be used as an effective indicator for users' security assessments.

==> figures/anova_cond_session.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Wed Sep 14 22:49:32 2016
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrr}
  \hline
 & Df & Sum Sq & Mean Sq & F value & Pr($>$F) \\ 
  \hline
cond      & 1 & 4994.18 & 4994.18 & 12.73 & 0.0009 \\ 
  Residuals & 41 & 16084.31 & 392.30 &  &  \\ 
  session      & 2 & 8570.89 & 4285.44 & 9.92 & 0.0001 \\ 
  cond:session & 2 & 9202.64 & 4601.32 & 10.65 & 0.0001 \\ 
  Residuals    & 82 & 35426.77 & 432.03 &  &  \\ 
   \hline
\end{tabular}
\end{table}


==> figures/anova_cond_task.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Wed Sep 14 22:49:32 2016
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrr}
  \hline
 & Df & Sum Sq & Mean Sq & F value & Pr($>$F) \\ 
  \hline
cond      & 1 & 4994.18 & 4994.18 & 12.73 & 0.0009 \\ 
  Residuals & 41 & 16084.31 & 392.30 &  &  \\ 
  task      & 2 & 8570.89 & 4285.44 & 9.92 & 0.0001 \\ 
  cond:task & 2 & 9202.64 & 4601.32 & 10.65 & 0.0001 \\ 
  Residuals1 & 82 & 35426.77 & 432.03 &  &  \\ 
   \hline
\end{tabular}
\end{table}


==> figures/chisq_between_session_S1.tex <==
($\chi^2(1)=0.11,p=1.000$)%

==> figures/chisq_between_session_S2.tex <==
($\chi^2(1)=0.79,p=1.000$)%

==> figures/chisq_session_ctrl_12.tex <==
($\chi^2(1)=2.00,p=1.000$)%

==> figures/chisq_session_ctrl_13.tex <==
($\chi^2(1)=6.15,p=0.118$)%

==> figures/chisq_session_ctrl_23.tex <==
($\chi^2(1)=0.79,p=1.000$)%

==> figures/chisq_session_expt_12.tex <==
($\chi^2(1)=3.62,p=0.513$)%

==> figures/chisq_website_ctrl_bank_db.tex <==
($\chi^2(1)=21.06,p<0.001$)%

==> figures/chisq_website_ctrl_bank_fb.tex <==
($\chi^2(1)=2.41,p=0.962$)%

==> figures/chisq_website_ctrl_fb_db.tex <==
($\chi^2(1)=10.20,p=0.011$)%

==> figures/chisq_website_expt_bank_db.tex <==
($\chi^2(1)=23.32,p<0.001$)%

==> figures/chisq_website_expt_bank_fb.tex <==
($\chi^2(1)=0.53,p=1.000$)%

==> figures/chisq_website_expt_fb_db.tex <==
($\chi^2(1)=15.99,p<0.001$)%

==> figures/complete_desc.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Thu Jul 28 14:15:31 2016
\begin{table}[ht]
\caption{Descriptive statistics for task completion times (in seconds).} 
\label{tab.time_desc_}
\begin{tabular}{lrrr}
  \hline
 & Stage 1 & Stage 2 & Stage 3 \\ 
  \hline
Test & 34.32 & 16.64 & 51.52 \\ 
  Control & 33.77 & 16.83 & 18.29 \\ 
  All & 34.05 & 16.73 & 34.90 \\ 
   \hline
\end{tabular}
\end{table}


==> figures/complete_desc_cond.tex <==
% latex table generated in R 3.2.4 by xtable 1.7-4 package
% Wed Jul  6 11:21:56 2016
\begin{table}[ht]
\caption{Descriptive statistics for task completion by condition.} 
\label{tab.complete_desc_cond}
\begin{tabular}{lrrr}
  \hline
 & Stage 1 & Stage 2 & Stage 3 \\ 
  \hline
Test & 3.0 & 2.0 & 2.0 \\ 
  Control & 3.0 & 3.0 & 3.0 \\ 
  All & 3.0 & 3.0 & 2.0 \\ 
   \hline
\end{tabular}
\end{table}


==> figures/complete_desc_website.tex <==
% latex table generated in R 3.2.4 by xtable 1.7-4 package
% Wed Jul  6 11:21:56 2016
\begin{table}[ht]
\caption{Descriptive statistics for task completion by website.} 
\label{tab.complete_desc_website}
\begin{tabular}{lrrr}
  \hline
 & Stage 1 & Stage 2 & Stage 3 \\ 
  \hline
Bank & 21 & 21 & 18 \\ 
  Dropbox & 17 & 12 &  9 \\ 
  Facebook & 19 & 20 & 17 \\ 
   \hline
\end{tabular}
\end{table}


==> figures/ttest_between_S1.tex <==
($t(21)=-0.15,p=1.000$)%

==> figures/ttest_between_S2.tex <==
($t(21)=0.14,p=1.000$)%

==> figures/ttest_between_X1.tex <==
($t(65)=-0.17,p=1.000$)%

==> figures/ttest_between_X2.tex <==
($t(65)=0.14,p=1.000$)%

==> figures/ttest_between_X3.tex <==
($t(65)=-3.32,p=0.013$)%

==> figures/ttest_c_S1S2.tex <==
($t(21)=6.01,p<0.001$)%

==> figures/ttest_c_S1S3.tex <==
($t(21)=3.52,p=0.019$)%

==> figures/ttest_c_S2S3.tex <==
($t(21)=-0.43,p=1.000$)%

==> figures/ttest_t_S1S2.tex <==
($t(21)=7.24,p<0.001$)%

==> figures/ttest_t_S1S3.tex <==
($t(21)=-1.74,p=0.868$)%

==> figures/ttest_t_S2S3.tex <==
($t(21)=-3.43,p=0.023$)%
